Limitations of Piecewise Linearity for Efficient Robustness Certification

Certified defenses against small-norm adversarial examples have received growing attention in recent years; though certified accuracies of state-of-the-art methods remain far below their non-robust counterparts, despite the fact that benchmark datasets have been shown to be well-separated at far larger radii than the literature generally attempts to certify. In this work, we offer insights that identify potential factors in this performance gap. Specifically, our analysis reveals that piecewise linearity imposes fundamental limitations on the tightness of leading certification techniques. These limitations are felt in practical terms as a greater need for capacity in models hoped to be certified efficiently. Moreover, this is in addition to the capacity necessary to learn a robust boundary, studied in prior work. However, we argue that addressing the limitations of piecewise linearity through scaling up model capacity may give rise to potential difficulties -- particularly regarding robust generalization -- therefore, we conclude by suggesting that developing smooth activation functions may be the way forward for advancing the performance of certified neural networks.

==> supplementary_sphere_approx.tex <==
% !TEX root=./main.tex

\section{Rounding Corners by Approximating Hyper-spheres}
\label{sec:sphere_approx}

% ... analyzing the decision boundary of a real-world example would be prohibitively expensive. Furthermore, the inability to solve the ``corner problem'' with reasonable capacity may lead the network to make other compromises that avoid corners but lead to sub-optimality in a way that is fundamentally caused by the same principle.

We consider the following thought experiment to provide some slightly more specific intuition regarding the additional capacity required to tightly certify regions near sharp ``corners'' in a piecewise-linear model's decision boundary.
As in Section~\ref{sec:corners}, we ...
The points for which certification is loose falls within the hypercube of width $\epsilon$, just opposite the corner.
The true robust frontier in this region is given by the intersecting orthant of the hypersphere of radius $\epsilon$...
In order to ... we must approximate this spherical orthant using linear hyperplanes that do not interse

